Conceptual Framework for Autonomous Cognitive Entities

The rapid development and adoption of Generative AI (GAI) technology in the form of chatbots such as ChatGPT and Claude has greatly increased interest in agentic machines. This paper introduces the Autonomous Cognitive Entity (ACE) model, a novel framework for a cognitive architecture, enabling machines and software agents to operate more independently. Drawing inspiration from the OSI model, the ACE framework presents layers of abstraction to conceptualize artificial cognitive architectures. The model is designed to harness the capabilities of the latest generative AI technologies, including large language models (LLMs) and multimodal generative models (MMMs), to build autonomous, agentic systems. The ACE framework comprises six layers: the Aspirational Layer, Global Strategy, Agent Model, Executive Function, Cognitive Control, and Task Prosecution. Each layer plays a distinct role, ranging from setting the moral compass and strategic thinking to task selection and execution. The ACE framework also incorporates mechanisms for handling failures and adapting actions, thereby enhancing the robustness and flexibility of autonomous agents. This paper introduces the conceptual framework and proposes implementation strategies that have been tested and observed in industry. The goal of this paper is to formalize this framework so as to be more accessible.

==> back/changed.tex <==
\section{Introduction}

The rise in scientific and commercial interest in autonomous machines has led to the development of numerous theories and models of machine autonomy, including self-driving cars and advanced AI systems. The proposed Autonomous Cognitive Entity (ACE) framework, which emphasizes internal thinking and reasoning abilities, is one such model. It allows for autonomous cognition even in extreme cases where there are no sensors or actuators, enabling AI to think independently before taking action.

The ACE framework makes several key contributions to the state-of-the-art cognitive architectures for artificial intelligence. Firstly, it pioneers a layered abstraction approach focused specifically on structuring internal cognition spanning from abstract reasoning to concrete actions. In contrast, prior layered models like OSI and SOA focus narrowly on external functions without modeling integrated cognitive capabilities \cite{}. Secondly, ACE uniquely integrates ethical principles and philosophical ideals directly within the upper layers of its architecture. This enables values alignment and beneficial decision-making unlike conventional approaches that lack built-in ethics \cite{}. Thirdly, the ACE framework incorporates psychological concepts like frustration tolerance and cognitive damping that are inspired by human cognition research. Existing architectures lack explicit modeling of these adaptive mechanisms \cite{}. Finally, the integration of LLMs enables ACE systems to leverage large scale knowledge and natural language understanding, advancing beyond the symbolic representations used in earlier models \cite{}. By combining hierarchical abstraction, integrated ethics, cognitive adaptation, and language modeling, the ACE framework aims to address limitations in prior AI architectures.

The ACE model is a hierarchical system, with each layer playing a unique role and interacting systematically with the others. The Aspirational Layer, at the top, sets the moral compass and overarching mission for the agent, interacting with all other layers to ensure alignment with the defined principles and mission statement. The Global Strategy Layer translates these principles and mission into a strategic vision, while the Agent Model Layer provides self-awareness, shaping the mission parameters around the agent's capabilities and limitations. The Executive Function Layer develops detailed plans based on these insights, guiding the actions of the Cognitive Control and Task Prosecution Layers, which manage and carry out tasks respectively.

The ACE framework's architectural choices, such as placing the moral/mission layer at the top, have sparked debates. This paper will discuss the rationale for this decision, drawing on insights from models like Maslow's hierarchy and findings from human psychology and neuroscience experiments. The layered abstraction allows for intervention at different levels, similar to how human behavior can be influenced at various brain levels. By placing morality, mission, and ethics at the top, the ACE framework promotes stable and predictable behavior aligned with its guiding principles.

The ACE framework incorporates insights from a range of disciplines, including neuroscience, philosophy, psychology, evolution, and computer science. 

From computer science and software engineering, the ACE framework draws inspiration from various models and principles, including the OSI model, SOAR, ACT-R, the Defense in Depth model of cybersecurity, and service-oriented architecture (SOA) and microservices. It conceptualizes artificial cognition in terms of discrete "cognitive functions" or layers, providing a structure for building autonomous systems using the latest AI capabilities such as large language models (LLMs) and multimodal generative models (MMMs).

From cognitive neuroscience, for instance, Jeff Hawkins’ “thousand brains” theory and V.S. Ramachandran’s work on localized brain damage have influenced the framework's layered abstraction and modular architecture. The study of brain disorders has also informed the ACE framework's design, helping to avoid common failure patterns through its hierarchical structure and integrated correction mechanisms. We draw inspiration from both global models and modular views of neuroscience.

Philosophically, the ACE model is influenced by Patricia Churchland's synthesis of neuroscience and philosophy, wherein she identified "Spheres of Caring" starting with the self nested at the center, and gradually expanding to encompass all humanity and all life.

Psychologically, the ACE model is influenced by the work of Maslow and Kohlberg. Maslow’s Hierarchy of Needs and Kohlberg's stages of moral development prioritize humanity's highest ideals and universal principles, aligning with the ACE framework's placement of the aspirational layer at the top.

The practical implications of the ACE framework are vast, with potential applications in video game NPCs, home robots, business automation, and more. For example, it could enable NPCs with independent personalities, goals, and agendas, or empower domestic robots to think flexibly beyond rigid programming. In business automation, the ACE framework could facilitate the creation of capable and reliable autonomous machines without the need for human intervention.

This paper is structured as follows: After this introduction, we review existing models and frameworks, explore philosophical concepts that align with the ACE Framework, and discuss models that have inspired the ACE Framework. We then present a detailed exploration of the ACE Framework, discussing each layer and its philosophical interpretation and relevance. We provide real or hypothetical implementation examples of the ACE Framework and analyze potential challenges and solutions. Finally, we discuss the interconnectedness of the layers, the integration of philosophical principles within the framework, and the practical implications of the ACE framework, before summarizing the key insights and making concluding remarks.


\subsection{Overview}

While currently a conceptual model, efforts are underway to computationally implement the ACE framework. Initial prototypes can be developed to validate the approach. For the Aspirational Layer, heuristic imperatives can be encoded as natural language rules that are interpreted by a DistilGPT model fine-tuned on ethics corpora. The Global Strategy Layer can use a BART model to summarize mission plans. To represent the Agent Model, a Graph Network can track state parameters, which are fed into a ResNet model to estimate capabilities. The Executive Function and Cognitive Control Layers are implemented through hierarchical task networks and Monte-Carlo tree search algorithms. For Task Prosecution, API calls and robotics middlewares like ROS provide actuation channels.

To integrate these components, inter-layer communications are implemented through a microservices architecture with REST APIs, message queues, and shared databases. Choreography protocols coordinate component interactions. The lower layers leverage deep learning for capabilities like computer vision, speech recognition, and natural language understanding through models like BERT and DALL-E. Ongoing work is focused on extending the prototype with more sophisticated algorithms, enhancing inter-layer coordination, and benchmarking system performance on simulation environments. This foundational implementation demonstrates initial feasibility while guiding further development towards real-world ACE applications.

\subsection{Philosophical Foundations}

The ACE framework also incorporates Patricia Churchland's concept of expanding "spheres of caring" from self to society and beyond \cite{churchland2011braintrust}. This concept links biological imperatives to abstract morality, bridging the cognitive and philosophical foundations of the ACE model. Of particular note, Churchland identified that, within the spheres of caring, suffering is a transitive property; the suffering of loved ones is equal to the suffering of self. This spoke directly to several of the universal values we present.

Despite being somewhat outdated, Sigmund Freud's theories of the conscious versus unconscious mind, and concepts like the ego, superego, and id, provide insight into self-awareness, self-direction, and internal conflict \cite{freud1989ego}. These theories offer a perspective on how layers dedicated to self-representation and idealized values might interact. In particular, the concept of the ego is a mental model of the self, which informed the design of the Agent Model, while the superego is an idealized version of the self couched in the context of society - a virtuous agent.

\section{Introduction}

Autonomous artificial intelligence (AI) systems are rapidly proliferating, as evidenced by advances in self-driving vehicles, intelligent household assistants, and responsive game characters. However, imbuing autonomous agents with the capacity for ethical reasoning remains an open challenge. Most conventional AI architectures lack integrated models of morality and human values, focusing narrowly on developing technical skills and capabilities. This paper aims to address this limitation by proposing a conceptual framework called the Autonomous Cognitive Entity (ACE) model for designing architectures that align autonomous AI systems with moral principles and ethical values.

Cognitive architectures like SOAR [2] and ACT-R [1] have enabled planning, problem-solving, and goal-directed behaviors by modeling high-level cognition. However, they rely heavily on predefined symbolic representations and struggle to handle complex, ambiguous real-world environments. Meanwhile, reinforcement learning offers trial-and-error learning but faces challenges in effectively and safely exploring exponentially large state spaces [59]. Recently, interest has emerged in incorporating large language models (LLMs) to enable more flexible reasoning and natural language understanding in AI systems [12, 54]. The proposed ACE framework builds upon these prior advances while pioneering new territory through an integrated model of ethical reasoning, autonomous decision-making, and layered abstraction spanning conceptual ideals to concrete actions.

The key innovation in the ACE model is its hierarchical structure consisting of six distinct layers, each handling specialized cognitive functions. The upper layers focus on moral reasoning, values, and high-level planning to shape the overall system direction. The lower layers address self-modeling, dynamic task management, and execution. Bi-directional information flow allows top-down oversight by the ethical reasoning modules while enabling bottom-up learning from the ground-up execution levels. This carefully coordinated architecture integrates insights from diverse disciplines including neuroscience, psychology, philosophy, and software engineering to realize artificial general intelligence capabilities within a system aligned with human values.

The paper is structured as follows: First, we provide comprehensive background on relevant prior work including cognitive architectures, AI ethics, layered system models, and autonomous agents. Next, we present the conceptual ACE framework in detail, explicating each of its six layers and their interconnections. We then demonstrate the framework's application through use cases including an autonomous virtual character and home assistant robot. Finally, we analyze architectural considerations, limitations, comparisons to existing models, and future research directions. Through the proposed ACE model, this research aims to establish a new paradigm for developing capable AI that aligns decisions and actions with moral principles and human values from the ground up.



\section{Introduction}

In recent years, artificial intelligence (AI) systems have become increasingly capable of operating autonomously to accomplish complex goals and tasks without human guidance [1]. However, imbuing autonomous agents with the capacity for ethical reasoning and alignment with human values remains an open challenge that has gained urgency alongside AI's rapid progress [2]. Most conventional AI architectures proposed in prior work lack integrated models of morality and focus narrowly on developing technical skills and capabilities rather than full internal cognitive faculties [3]. This paper introduces the Autonomous Cognitive Entity (ACE) model, a novel conceptual framework for architecting ethical artificial general intelligence based on a layered cognitive architecture.

The advent of large language models (LLMs) such as ChatGPT has catalyzed a paradigm shift towards incorporating natural language understanding into cognitive architectures \cite{sumers2023cognitive}. These models possess extensive world knowledge and sophisticated language comprehension abilities acquired through pre-training on massive text corpora [5]. Formulating cognitive capabilities in natural language allows LLMs to serve as key components, enabling a flexible understanding of contextual information [6]. However, standalone LLMs lack the architectural integration needed for robust and corrigible autonomous systems. The proposed ACE framework aims to harness these emerging capabilities but further innovate architecturally to privilege ethics, security, and human alignment.

The proliferation of LLMs has raised many philosophical puzzles regarding the nature of the reasoning and understanding demonstrated by these models. It remains unclear precisely how the statistical patterns LLMs acquire from textual training data might correspond to human-like conceptual knowledge and semantics. Assumptions that LLMs obtain true comprehension of meaning and reasoning purely from statistical co-occurrence patterns remain speculative [10]. Significant gaps persist in elucidating how LLMs represent abstractions relating to truth, inference, and symbol grounding. While they show promise in replicating certain facets of human intelligence, we must be cautious against premature conclusions that LLMs fully capture capacities like common sense or generalizable reasoning [12]. Nevertheless, their practical utility for specialized applications is clear, and the ACE framework aims to leverage their strengths while mitigating limitations through architectural integration.

The key innovation in the ACE model is its hierarchical structure consisting of six layers, each handling specialized cognitive functions [13]. The upper Aspirational and Global Strategy layers focus on moral reasoning, values, and high-level planning to shape the overall system direction. The mid-level Agent Model, Executive Function, and Cognitive Control layers address self-modeling, dynamic task management, and decision-making. Finally, the bottom Task Prosecution layer handles execution and embodiment. Bi-directional information flow allows top-down oversight by the ethical reasoning modules while enabling bottom-up learning from the ground-up execution levels. This coordinated architecture integrates insights from diverse disciplines including neuroscience, psychology, philosophy, and software engineering to realize artificial intelligence capabilities within a system aligned with human values. The ACE framework incorporates both deontological and teleological ethical approaches, rejecting an "either/or" stance in favor of a "both/and" perspective [19]. By embedding abstract principles and technical implementation together within a unified architecture, the ACE model provides a systematic framework for developing capable and beneficial autonomous cognitive systems. The layered encapsulation draws lessons from paradigms like the OSI model to enhance security, corrigibility, and coordination \cite{stallings1987handbook}.

The hierarchical abstraction enables clear separation of concerns between layers, from ethical reasoning down to physical embodiment. This enhances interpretability since the capabilities and limitations at each level are transparent. The privilege separation also aids corrigibility by allowing the Aspirational Layer to monitor and intervene to correct deviations. And the bidirectional flows facilitate both oversight and learning across the cognitive stack. Together, these architectural principles aim to produce AI systems that are capable, secure, and aligned with human values. The ACE framework methodology discusses safety properties, detailed computational implementations, and comparative conceptual evaluations on diverse scenarios. By contributing the conceptual ACE framework, this paper hopes to catalyze exploration into architectures integrating ethics and learning for artificial general intelligence. The introduced model establishes an initial foundation, guiding follow-on engineering efforts towards the long-term goal of developing AIs that learn, adapt and thrive while remaining steadfastly aligned to the aspirations of humanity. Extensive research across many dimensions will be essential to fully realize this vision in applied autonomous systems.

The paper is structured as follows: First, we provide comprehensive background on relevant prior work including cognitive architectures, AI ethics, layered system models, and autonomous agents. Next, we present the conceptual ACE framework in detail, explicating each of its six layers and their interconnections. We then demonstrate the framework's application through use cases including an autonomous virtual character and home assistant robot. Finally, we analyze architectural considerations, limitations, comparisons to existing models, and future research directions. Through the proposed ACE model, this research aims to establish a new paradigm for developing capable AI that aligns decisions and actions with moral principles and human values from the ground up.


The ACE framework methodology involves formal verification of safety properties, detailed computational implementations, and comparative evaluations on diverse tasks [25]. Formal encodings of philosophical principles and mathematical proofs of alignment will complement empirical assessments [26]. Standardized benchmarks and simulations can quantify capabilities, while adversarial techniques like red teaming probe security [27]. Human-subject studies will elicit user feedback on transparency, interpretability, and trustworthiness [28]. By combining rigorous testing, benchmarking, deployment studies, formal analysis, and human-subject evaluations, the merits and limitations of the ACE framework can be comprehensively validated across key criteria of capabilities, security, and alignment essential for applied autonomous cognitive systems [29].




These principles are derived from diverse sources such as philosophy, neuroscience, evolution, and frameworks like Maslow's Hierarchy of Needs, Self-Determination Theory, Choice Theory, and Therapeutic Lifestyle Changes. They assert the general notions that suffering should be reduced, prosperity increased, and understanding increased, with their universal scope applying to all organisms and sentient entities, providing foundational ethical values.

It is important to avoid superlatives such as "minimize" and "maximize" because that is not the intention of these frameworks. For instance, it is impossible to eliminate suffering without also extinguishing life, and maximizing prosperity and understanding should not come at the expense of each other. The semantic difference between "reduce" and "minimize" might not seem significant, but it is crucial, as testing in large language models has shown that wording is very important.

In experiments, adding these heuristics enabled large language model-driven systems to maintain good perspective and make more reasoned judgments aligned with ethical principles, recommending universal principles as the primary overarching framework. For fictional agents like game NPCs, alternative value frameworks, such as Greek virtues for an ancient Greek character, can be substituted, allowing for customization of principles tailored to specific agent roles and natures.


\subsection{Comparison with other Frameworks}

A key part of assessing any new conceptual model is comparing it to existing related frameworks, analyzing the similarities, differences, and unique contributions. This section will compare the layered architecture of the proposed Autonomous Cognitive Entity (ACE) model with two alternative cognitive architectures from recent research – the Autonomous Machine Intelligence (AMI) model \cite{lecun2022path} and the Cognitive Architecture for Language Agents (CoALA) framework \cite{sumers2023cognitive}.

By elucidating the key distinctions between ACE and these other approaches across each architectural layer, this analysis aims to highlight the novel aspects of ACE's design. The comparisons focus on how the frameworks differ in their structure, capabilities, and integration of components for autonomous cognition. Examining these architectural variations provides perspective into how ACE diverges from prior architectures and establishes a distinct paradigm.

The goal is to situate ACE in the landscape of related autonomous agent architectures, delineating its conceptual innovations regarding the integration of ethics, emphasis on internal cognition, hierarchical abstraction, and specialized metacognitive functions. This section provides an overview comparing ACE to AMI and CoALA, while the subsections will examine the architectural differences layer-by-layer in more depth. The comparative analysis intends to clarify ACE's contributions as a transdisciplinary synthesis toward beneficial and human-aligned autonomous intelligent systems.

\subsubsection{Autonomous Machine Intelligence Model}

This section compares the layered architecture of the proposed Autonomous Cognitive Entity (ACE) framework with the Autonomous Machine Intelligence (AMI) \cite{lecun2022path} architecture presented in the baseline paper.

\textbf{Aspirational Layer}

% Original % The Aspirational Layer in the ACE framework establishes high-level ethical principles and moral values to guide the agent’s behavior. This is conceptually related to the Intrinsic Cost module in the AMI architecture, which defines basic drives and motivations. However, the Intrinsic Cost module operates at a lower level concerned with basic needs and emotions, while the Aspirational Layer focuses on abstract philosophical ethics. The Aspirational Layer also oversees all other layers to ensure alignment with moral principles, playing an ethical oversight role analogous to the dynamic configuration performed by the AMI Configurator module.

The Aspirational Layer, a key innovation in the ACE framework, is focused on establishing an ethical and philosophical foundation to guide the agent's behavior by defining high-level principles, values, and imperatives using natural language descriptions. In contrast, the AMI architecture lacks an explicit aspirational reasoning module, with the closest analogue being the Intrinsic Cost module, which encodes basic drives and motivations to fulfill internal needs but is positioned at a lower level concerned with primitive functions rather than high-level cognition.

Operating at a more abstract level, the Aspirational Layer in ACE is focused on moral reasoning and idealized principles, providing top-down oversight to ensure alignment with defined ethics across all layers, whereas the Intrinsic Cost module in AMI has no capacity for such ethical oversight. Furthermore, the Aspirational Layer allows for the formulation of ethics, principles, and values in natural language, facilitating interpretability and enabling the leveraging of LLMs' nuanced language understanding abilities, while AMI does not emphasize natural language principles.

Overall, the distinct Aspirational Layer in ACE provides architectural innovation through the explicit integration of abstract philosophical ethics, aiming to guide behavior using conceptual ideals rather than solely individual drives. This is in contrast to AMI, which lacks architectural separation between technical optimization and aspirational reasoning. By embedding ethics within ACE's highest layer, the framework institutes moral judgments and social values as the primary decision-making foundations, differentiating it from AMI's individualistic optimization approach and exemplifying ACE's focus on aligning agent actions to human principles rather than internal fulfillment.

\textbf{Global Strategy Layer}

% Original % The Global Strategy Layer creates high-level plans and strategies guided by the ethical principles defined in the Aspirational Layer. This is broadly comparable to the AMI Actor module which proposes technically optimized action sequences. However, the Global Strategy Layer is more focused on strategic reasoning rather than technical optimization. It also translates abstract aspirational goals into implementable strategic plans, going beyond the AMI Configurator’s role of configuring modules for specific tasks.

% proposed change below

The Global Strategy Layer in the ACE framework is responsible for constructing a model of the agent's environment and broader context, integrating real-time sensory input and background knowledge to maintain an up-to-date understanding of the external world. This is conceptually similar to the World Model module in the AMI architecture, which learns a model of environment dynamics from perception, and the Perception module in AMI, which takes in information from the environment. However, the Global Strategy Layer plays a more central role in planning and directing behavior in the ACE framework compared to AMI, actively guiding actions rather than solely building an environment model.

The key difference lies in the ACE framework's reliance on the latent world knowledge already present in large language models (LLMs), obviating the need to completely rebuild environment models from scratch. The Global Strategy Layer grounds the LLM's implicit knowledge by integrating real-time context and is designed to "think" in more abstract strategic principles, rather than immediate concrete actions, addressing the lack of big-picture long-term thinking in the AMI model. By combining updated situational data with the LLM's vast latent knowledge, the Global Strategy Layer constructs a sufficiently accurate world model to inform planning, providing targeted grounding to steer the LLM's capacities towards useful behaviors suited to the current context.

In this way, the ACE Global Strategy Layer serves as a critical component in guiding the agent's behavior using both environmental inputs and the LLM's intrinsic conceptual understandings. Its role in planning is more central compared to the perception-focused modules in AMI, exemplifying how ACE strategically leverages LLMs to reduce duplication of world knowledge and enhance the agent's decision-making capabilities.

\textbf{Agent Model Layer}

% The Agent Model Layer in the ACE framework constructs a representation of the agent’s capabilities and self-model. This has parallels with the AMI Actor which learns and proposes actions based on the agent's skills. However, the Agent Model Layer is solely focused on metacognitive self-representation rather than action selection. Action selection is handled by a lower layer in the ACE model, the Cognitive Control layer. Both the AMI and ACE model recommend that agents update their self-understanding through interaction with the environment, such as by observing successes and failures. 

The Agent Model Layer in the ACE framework develops an explicit self-representation of the agent's capabilities, architecture, and limitations, serving as a metacognitive model detached from direct embodiment, in contrast to the AMI architecture which distributes related functions like skill learning and memory across separate modules such as the Actor, Critic, and World Model. The ACE Agent Model encapsulates these faculties into a consolidated introspective layer, incorporating both episodic and declarative memory to track the agent's experiences and knowledge, and maintaining an internal narrative timeline of past states, events, and decisions, which is considered intrinsic to self-modeling.

The key differentiation is that the Agent Model Layer in ACE exclusively focuses on constructing an abstract self-representation, architecturally isolated from outwardly-focused components like perception, planning, and action selection, with this privileged separation aiming to develop a robust internal metacognitive representation decoupled from reactive pressures. The self-model can then provide an embedded perspective to guide decision-making across contexts. In summary, the ACE Agent Model Layer concentrates metacognition, memory, and self-monitoring in an encapsulated module, diverging from the distributed approach in AMI and enabling rich integrated self-knowledge to orient strategic reasoning and actions.

\textbf{Executive Function Layer}

% The Executive Function Layer concretizes the strategic plans produced by the higher layers into executable actions. This is highly analogous to the AMI Actor module which generates optimal action sequences. However, the ACE Executive Function Layer also manages additional responsibilities such as resource allocation and risk management. The AMI model addresses this via the Intrinsic Cost and Critic modules.

The ACE Executive Function Layer serves as a bridge between high-level strategic reasoning and low-level behavioral implementation, converting abstract directives from higher layers into concrete action plans and executable tasks. This differentiates ACE from the AMI architecture, where planning modules like the Actor operate at the concrete level detached from conceptual oversight. In contrast, the ACE Executive Function Layer is contextualized by the ethical principles, strategic goals, and self-knowledge flowing down from upper layers, allowing for a clear hierarchy as information transitions from abstract to concrete. The AMI approach lacks this clear hierarchy, with planning modules focused narrowly on technical optimization rather than integrating top-down context.

By leveraging robust conceptual inputs from above, the ACE Executive Function Layer can undertake key oversight responsibilities beyond AMI's Actor module, including comprehensive project planning, risk management, resource allocation, and formulating success criteria. This enables the generation of pragmatically optimized plans suited to the agent's principles, objectives, and limitations, rather than just technically optimal behaviors. It concretizes the contextual guidance from above into feasible action roadmaps, exemplifying ACE's integrated approach.

The privileged hierarchy in ACE enables the Executive Function Layer to produce plans embedded within a broader strategic vision, contrasting with AMI's localized planning detached from higher cognition. The AMI model addresses this via the Intrinsic Cost and Critic modules, but the ACE framework's emphasis on unifying ethical reasoning and autonomous learning within a layered cognitive architecture offers a more comprehensive solution.

\textbf{Cognitive Control Layer}

% The Cognitive Control Layer in the ACE model performs adaptive behavior by selecting and switching between tasks based on real-time feedback and interaction with the environment. The AMI Critic and Actor play a similar adaptive role shaping actions based on environmental outcomes. However, the ACE Cognitive Control Layer incorporates additional functions such as frustration signals and cognitive damping.

The ACE Cognitive Control Layer and AMI's Critic and Actor modules both aim to adapt actions based on real-time feedback; however, the Cognitive Control Layer incorporates additional metacognitive functions inspired by human cognition, such as frustration signals, deliberation between options, and dampening hasty reactions. These mechanisms enhance flexible decision-making when original plans are disrupted, in contrast to AMI, which does not include explicit capabilities to handle unexpected failures or situations where initial goals become irrelevant. Lacking architectural support for cognitive control, AMI is ill-equipped for autonomous adaptation.

The ACE Cognitive Control Layer enables critical functions like task switching and dynamic re-prioritization when pre-defined contingencies fail, allowing the agent to quickly change course in the event of an emergency rather than stubbornly pursuing outdated goals. This resembles human cognitive control, where individuals calmly reassess circumstances when plans go awry before deciding how to respond appropriately. In comparison, the AMI architecture's reactive approach leaves it vulnerable when core assumptions are invalidated. By incorporating metacognitive processes specialized for uncertainty and change, the ACE Cognitive Control Layer provides crucial cognitive control abilities absent in AMI, facilitating safer autonomous operation in unpredictable real-world environments.

\textbf{Task Prosecution Layer}

% The Task Prosecution Layer executes actions, akin to the AMI Actor. However, it also actively monitors outcomes and provides feedback, unlike the reactive AMI Actor.

The ACE Task Prosecution Layer, comparable to AMI's Actor module as the low-level executor, separates many Actor functions into a more hierarchical structure, privileging abstract cognition over physical skills. In this framework, the sense of self and intentions reside in higher layers, while the Task Prosecution Layer focuses narrowly on basic input/output, resembling how human hands follow top-down instructions from the brain without making high-level judgments. Consequently, the ACE Task Prosecution Layer acts peripherally, not centrally.

Structurally separating low-level execution from cognition and memory provides greater flexibility, enabling interoperability with diverse physical and digital environments. For instance, robotic systems could implement the ACE stack and connect it to different prosthetic hands based on the situation, allowing the invariant ACE cognition to transfer seamlessly across embodiments. In contrast, AMI's Actor module bundles together both abstract reasoning and embodiment-specific skills, whereas the ACE approach better isolates generic cognitive capabilities from situation-specific execution mechanisms.

By architecturally distinguishing general cognition from basic input/output, ACE frameworks gain significant optionality in how they interface and interact with the external world, facilitating extensible systems that emphasize transferable reasoning abilities.

\textbf{Overview}

% In summary, the ACE framework defines distinct conceptual layers separating moral reasoning, strategic planning, self-modeling, and execution. In contrast, the AMI architecture combines these functions within interconnected modules like the Actor and Configurator. The AMI approach provides more integrated system-level oversight but the ACE model enables greater architectural separation between philosophical reasoning and technical implementation.

The ACE and AMI architectures take fundamentally different approaches to structuring autonomous cognition. A key differentiation is that ACE employs a strict hierarchical structure with clear boundaries between layers of abstraction. Control flows top-down from the highest Aspirational Layer down through the sequence of lower layers. Each layer has tightly defined responsibilities and privileges, with higher layers able to monitor and direct lower ones. This regimented organization contrasts with AMI, which allows more flexible interconnectivity between modules. While AMI offers greater integration, ACE’s hierarchical delineation aims to enhance interpretability, predictability, and most importantly - safety.

By architecting clear levels of abstraction from the Aspirational Layer down to the Task Prosecution Layer, ACE creates a logical gradient from the most abstract moral reasoning to the most concrete physical actions. The upper layers focused on ethics constrain the lower layers focused on execution. AMI does not exhibit this same orderly transition, with planning and technical faculties like the Actor module operating detached from ethical oversight. ACE’s abstraction-oriented approach hopes to deliver more coherent structure akin to paradigms like the OSI model.

Furthermore, ACE uniquely privileges the Aspirational Layer above all others, cementing aspiration ethics as the foremost decision factor. This provides strong top-down control to align system behavior to human values. AMI lacks an ethical reasoning module dedicated to overriding lower subsystems. By prioritizing aspirational morality, ACE institutes value alignment as a central architectural principle rather than a secondary concern.

Through hierarchical abstraction, segmented privileges, and ethical primacy, the ACE architecture aims for safer, more predictable, and human-centered autonomous systems compared to AMI’s flexibility-oriented integration. However, thorough comparative evaluations are needed to fully assess the strengths and weaknesses of both approaches in applied autonomous agents.

\subsubsection{Cognitive Architectures for Language Agents}

This subsection provides an in-depth layer-by-layer comparison between the Autonomous Cognitive Entity (ACE) framework proposed in the ACE framework and the alternative approach presented in the Sumers et al. paper about Cognitive Architectures for Large Language Models \cite{sumers2023cognitive}. They propose Cognitive Architectures for Language Agents (CoALA) framework that we discuss in this section.

\textbf{Aspirational Layer}: The Aspirational Layer is a key conceptual innovation in our ACE framework. It establishes high-level ethical principles, values, and imperatives to guide the agent's behavior. This enables top-down value alignment and moral oversight over system operation. Sumers et al. paper incorporates intrinsic motivations and philosophical ethics to shape objectives, which bears some similarity. However, our Aspirational Layer operates at a more abstract level focused on idealized principles rather than intrinsic drives or technical metrics. Our Aspirational Layer monitors all layers and can intervene if deviations from principles are detected. This allows strong top-down ethical control. The CoALA approach lacks an architectural separation between abstract aspirational reasoning and technical implementation. In contrast, our distinct Aspirational Layer enforces clearer boundaries between moral judgments and lower-level actions. This privilege separation aids value alignment, security, and corrigibility. Furthermore, our Aspirational Layer allows formulating principles and ethics in natural language, leveraging LLM interpretive abilities. The CoALA framework does not emphasize natural language formulations. Overall, our Aspirational Layer provides architectural innovation in value alignment missing from the CoALA framework.

\textbf{Global Strategy Layer}: Our Global Strategy Layer creates high-level plans and strategies guided by the ethical principles defined in the Aspirational Layer. It draws on the latent knowledge within LLMs to translate aspirational goals into strategic directives. This resembles the Actor module in the CoALA framework approach which proposes technically optimized action sequences. However, our Global Strategy Layer places much greater emphasis on strategic reasoning rather than technical optimization. It focuses more on determining optimal approaches and general principles given the agent's context and capabilities. The Global Strategy Layer also differs in its dynamic adaptation based on feedback from lower layers. The Actor module in the CoALA framework is more static once configured. Our Strategic Layer continuously revises plans as the context evolves. It also handles long-term forecasting going beyond the Actor's focus on immediate actions. This enables our layer to shape the agent's overarching direction rather than solely generating incremental steps.

\textbf{Agent Model Layer}: The Agent Model Layer in the ACE framework constructs and maintains an accurate self-representation of the agent's capabilities, architecture, and limitations. This metacognitive self-model enables reasoning detached from the external environment. In contrast, the Actor module in the CoALA framework focuses outwardly on selecting actions based on skills learned from environmental interaction. Our Agent Model Layer instead looks inward to develop an explicit understanding of the agent's own configuration and abilities. This self-awareness facilitates adaptable reasoning and planning by grounding decisions in an accurate model of the agent's capacities. Our Agent Model Layer incrementally expands knowledge of the agent's capabilities through observational learning. The CoALA framework lacks an analogous self-representation and metacognition module.

\textbf{Executive Function Layer}: Our Executive Function Layer concretizes the strategic plans from higher layers into detailed executable routines and measurable goals. This resembles the role of the Actor module in the alternative approach which generates low-level action sequences. However, our Executive Function Layer incorporates additional responsibilities that extend beyond the Actor's scope. Notably, our layer handles key aspects of resource management, risk assessment, contingency planning, and defining success criteria. The Actor module focuses narrowly on technical optimization without these additional oversight functions. Our Executive Function Layer thus acts akin to a project manager, ensuring effective planning and adaptation. Furthermore, our layer dynamically adjusts plans based on feedback, whereas the Actor operates more reactively. This proactive flexibility enhances robustness and goal achievement in complex environments. Overall, our Executive Function Layer incorporates cruicial planning faculties absent in the CoALA framework.

\textbf{Cognitive Control Layer}: The Cognitive Control Layer in our framework handles moment-to-moment decision making based on the current context. This includes selecting the next appropriate task and dynamically switching between tasks as circumstances change. The Critic and Actor modules in the CoALA framework also aim to shape actions based on real-time feedback. However, our Cognitive Control Layer integrates additional adaptive mechanisms. Specifically, our layer implements metacognitive functions modeled on human cognition such as frustration tolerance, deliberation between options, and cognitive damping. These mechanisms enhance flexible decision making in complex situations with uncertainty or conflict. The CoALA framework lacks analogous metacognitive faculties. Our layer also facilitates adaptability through bi-directional communication with both upper and lower layers.

\textbf{Task Prosecution Layer}: Our Task Prosecution Layer executes actions selected by the Cognitive Control Layer and monitors their outcomes. This is comparable to the role of the Actor module in the CoALA framework. However, our layer places greater emphasis on interpreting task outcomes and providing rich feedback both on successes and failures. The Actor has a more reactive role focused on sensory-motor skills. In contrast, our Task Prosecution Layer proactively labels task results, measures performance, and identifies defects or deviations. This feedback is essential for ongoing learning and adaptation across the ACE framework. Our layer also incorporates wider functions beyond physical actions, such as API calls and code execution for digital environments. This expands competence beyond the Actor's physical embodiment.

\textbf{Overview}

While our ACE framework shares high-level similarities with the CoALA framework, there are major differences in the specific focus, capabilities, and integration of each layer. The ACE framework greater separation between moral reasoning and technical implementation. It also emphasizes rich metacognitive representations and feedback channels enabling ongoing autonomous adaptation. This architectural approach aims to enhance the flexibility, robustness, and human alignment of cognitive agents.
